Analyzing Regrettable Communications on Twitter: Characterizing Deleted Tweets and Their Authors

Over 500 million tweets are posted in Twitter each day, out of which about 11% tweets are deleted by the users posting them. This phenomenon of widespread deletion of tweets leads to a number of questions: what kind of content posted by users makes them want to delete them later? %Are all users equally active in deleting their tweets or Are users of certain predispositions more likely to post regrettable tweets, deleting them later? In this paper we provide a detailed characterization of tweets posted and then later deleted by their authors. We collected tweets from over 200 thousand Twitter users during a period of four weeks. Our characterization shows significant personality differences between users who delete their tweets and those who do not. We find that users who delete their tweets are more likely to be extroverted and neurotic while being less conscientious. Also, we find that deleted tweets while containing less information and being less conversational, contain significant indications of regrettable content. Since users of online communication do not have instant social cues (like listener's body language) to gauge the impact of their words, they are often delayed in employing repair strategies. Finally, we build a classifier which takes textual, contextual, as well as user features to predict if a tweet will be deleted or not. The classifier achieves a F1-score of 0.78 and the precision increases when we consider response features of the tweets.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

% == Socio-linguistic insights (what we learn from the study) ==

% the second paragraph of the present Conclusion —

% personality traits of deleters and non-deleters are indeed different human
% beings are bad at understanding why others deleted tweets, but ML classifiers
% can predict with more accuracy similar to offline world, audience response is
% correlated with tweet deletions

% == What Twitter (and ultimately Twitter users) can benefit from the study ==

% Studying tweet deletions (or lack of them) might be a good way to figure out
% personality traits of users, which will improve lot of other applications like
% personalised recommendations

% Simple tools to edit tweets can be provided — will do away with need for
% superficial deletions (which are the majority)

% Specifically, depending on the personality traits of users, tools can be
% deployed to warn them about possible posting of regrettable content. Whether or
% not a user would like such a tool needs to be figured out as well, e.g., users
% who have to repeatedly delete tweets might actually like such tools

% Tools for warning users about possible regrettable content need to be
% personalised as well, e.g., the classifier designed in this study can be used
% for new users, and the classifier will be refined / personalised based on the
% tweets that the user actually deletes / does not post after being warned

% Such tools can also warn users if initial responses to a tweet are negative, so
% that the user can quickly delete post if necessary and thus limit the damage

% All these can help to improve the user experience on Twitter

% == Unanswered questions ==

% if a tweet has received significant negative response, what should be done with
% the responses even if the tweet is deleted? should responses be deleted as well,
% or at least the users who responded notified that the original tweet has been
% deleted? if the responses remain in the system, they lead to potential privacy
% leaks as shown by mondal et al.

\begin{NewText}

Our analysis has shown that
it is definitely possible to predict
the possibility of a tweet being deleted
in the future with decent accuracy.
However, when developing systems
trying to nudge users towards better privacy
a number of factors need to be taken into account.

% Existing works dont account for user differences
% Classifers built are impersonal
% Whether to delete a tweet or not is deeply personal
% User personality more than anything else decides if a tweet will be deleted or not.
\textbf{One size doesn't fit all:}
Earlier works~\cite{petrovic-unpub00,zhou-www15} trying to predict the
possibility of a tweet getting deleted
focused only on the content of the tweet itself.
We note that,
whether the author of a tweet finds a tweet to be regrettable or not,
depends deeply on the author herself.
Thus, it is imperative for developers,
trying to create systems that nudge users towards better choices,
to develop personalized classifiers
which take into account personality and behavior of the user
when making such predictions.

% Number of works on nudging
% Systems need be careful when nudging users
% Nagging: Google Mail goggles
% Designing systems need be unobtrusive
\textbf{Nudges are good, nagging is bad:}
Wang et al.~\cite{wang-chi14} in their study
to nudge users towards better usage of privacy features
noted that
about half the users in their survey
held negative or indifferent attitudes
towards the widgets presented to help them.
A similar response could be seen
in users of Google Mail Goggles,%
\footnote{%
Mail Goggles~\cite{mail-goggles} was an optional widget
available with Google Mail during October 2008 to May 2012.
When enabled, Mail Goggle users
were required to answer simple math questions
to demonstrate cognitive abilities
before it allowed them to send emails.
The service was intended to stop drunk email late at night.}
many of whom found it annoying rather than helpful.
We hypothesize that whether a user finds it useful
to trade off ease of use for increased privacy
depends heavily on the personality
of the user as well as the importance the user places
on the requirement of privacy.
Thus, it is important for system designers
to not only understand the personality of the users
being exposed to such systems
but also to educate and convince them
of the problems their system is designed to solve.
Otherwise, systems of these categories
run the risk of being mostly ignored.

% 14\% superficial deletions
% Delete and Create vs Edit
%   http://www.wired.com/2013/04/what-twitter-needs/
% Pros:
%   Easier to implement
%   Higher accountability
% Cons:
%   Losing responses
%   Misuse and spam
\textbf{Deletion as an editing tool:}
Twitter as of date doesn't provide a method to edit tweets.
The result of which is that
any user trying to edit any of her tweets
needs to first delete the offending tweet
and compose a new one.
We find in our dataset that about 14\% of the deletions
are superficial, that is the tweets were deleted by their
authors to post a fixed and slightly modified version of the
original tweet.
While there has been considerable demand for editing
facility from celebrities and popular media,%
\footnote{\url{http://www.wired.com/2013/04/what-twitter-needs/}}
allowing users to edit tweets definitely has its pros and cons.
On the con side,
deleting and re-composing the tweet is often
a problem for users
as the process severs the links
between the tweet and its responses.
On the other hand,
allowing users to edit tweets
can produce numerous forms of gaming systems
where a user of a highly retweeted tweet can
change the content of the original tweet
which may not be in agreement with the users who
did the retweeting.

\end{NewText}


==> tables/bad-sources-list.tex <==
\begin{table}
\centering
\begin{tabu} to \linewidth{@{}lr@{}}
\toprule

Client & \% Tweets \\

\midrule

Twittascope   & 277724 / 180003862 0.154288
RoundTeam     & 262389
IFTTT         & 203299
Google        & 164705
dlvr.it       & 129954
Buffer        & 120516
fllwrs        & 96279
Ask.fm        & 85747
twittbot.net  & 81020
WordPress.com & 80763

\bottomrule
\end{tabu}
\caption{List of top 10 specialized Twitter clients
removed from our analysis,
from the deleted tweet set and the regular tweet set.}
\label{tab:bad-sources-list}
\end{table}



==> tables/dataset-stats-clean.tex <==
\begin{table}
\centering
\begin{tabu} to \linewidth{@{}lr@{}}
\toprule

\# Tweets posted & 17,147,771 \\
\# Tweets deleted & 1,210,434 (7.05\%) \\
\# Users who posted at-least 1 tweet & 194,495 \\
\# Users who deleted at-least 1 tweet & 91,785 (47.19\%) \\

\bottomrule
\end{tabu}
\caption{Total number of tweets posted and deleted by users in our dataset,
\emph{after} removal of non-english tweets, automated tweets, retweets,
and superficial deletions.}
\label{tab:dataset-stats-clean}
\end{table}



==> tables/dataset-stats.tex <==
\begin{table}
\centering
\begin{tabu} to \linewidth{@{}lr@{}}
\toprule

\# Tweets posted & 43,119,286 \\
\# Tweets deleted & 4,793,101 (11.11\%) \\
\# Users who posted at-least 1 tweet & 214,471 \\
\# Users who deleted at-least 1 tweet & 152,591 (71.14\%) \\

\bottomrule
\end{tabu}
\caption{Total number of tweets posted and deleted by users in our dataset,
\emph{before} removal of non-english tweets, automated tweets, retweets,
and superficial deletions.}
\label{tab:dataset-stats}
\end{table}

% Tweet rate our dataset
% 43119286 / 214471
% 201.049494

% Tweet rate Almuhimedi dataset
% 67295171 / 222185 * 4
% 1208.0


==> tables/del-prot.tex <==
\begin{table}[t]
\centering
\begin{tabu}{@{}lrr@{}}
\toprule

& Deleted Tweet Set & Regular Tweet Set \\

\midrule

% \# Suspended & 49,621 (2.66\%) & 46,254  (1.89\%) \\
\# Deleted   & 76,230 (4.10\%) & 56,623  (2.32\%) \\
\# Protected & 85,634 (4.60\%) & 102,161 (4.18\%) \\
% \# Unsafe    & 13,387 (0.72\%) & 6,153   (0.25\%) \\

\bottomrule
\end{tabu}

\caption{Number of users in the two datasets,
  % who had their accounts suspended,
  who have deleted their accounts voluntarily,
  who have made their account protected,
  % and who have posted at-least one unsafe url.
  Numbers within parenthesis
  are the percentage of users of given type.}
\label{tab:del-prot}
\end{table}

% 49621 / 1859452.0 = 2.668582
% 46254  / 2440561.0 = 1.89522
% Fisher-Exact: OR = 1.41925, p = 0

% 76230 / 1859452.0 = 4.099595
% 56623  / 2440561.0 = 2.320081
% Fisher-Exact: OR = 1.79979, p = 0

% 85634 / 1859452.0 = 4.605335
% 102161 / 2440561.0 = 4.185964
% Fisher-Exact: OR = 1.10502, p = 2.8273e-98

% 13387 / 1859452.0 = 0.719943
% 6153   / 2440561.0 = 0.252114
% Fisher-Exact: OR = 2.86908, p = 0


==> tables/del_liwc_corr.tex <==
Category  :   r        p(r=0)     rho      p(rho=0)   mic
-----------------------------------------------------------
you       :   0.082    (9e-132)   0.098    (2e-186)   0.073
article   :  -0.019    (1e-08)   -0.048    (5e-47)    0.064
auxverb   :   0.030    (8e-20)    0.041    (4e-34)    0.056
future    :  -0.025    (9e-14)   -0.082    (8e-133)   0.113
negate    :   0.055    (1e-59)    0.047    (2e-44)    0.082
quant     :   0.031    (5e-21)    0.015    (2e-06)    0.083
social    :   0.084    (1e-137)   0.091    (5e-161)   0.058
family    :   0.021    (1e-10)   -0.060    (3e-72)    0.132
humans    :   0.067    (5e-88)    0.041    (2e-34)    0.103
negemo    :   0.066    (5e-86)    0.067    (4e-89)    0.070
sad       :   0.067    (6e-90)    0.038    (2e-29)    0.127
cogmech   :   0.034    (6e-25)    0.032    (7e-22)    0.055
cause     :   0.000    (9e-01)   -0.030    (1e-19)    0.087
discrep   :   0.042    (1e-35)    0.024    (2e-13)    0.084
certain   :   0.067    (6e-89)    0.059    (5e-69)    0.093
hear      :  -0.004    (1e-01)   -0.091    (7e-163)   0.140
feel      :   0.030    (1e-19)   -0.017    (4e-07)    0.138
bio       :   0.059    (5e-70)    0.069    (7e-93)    0.070
body      :   0.036    (1e-26)    0.005    (1e-01)    0.108
health    :   0.029    (9e-18)   -0.017    (3e-07)    0.133
ingest    :  -0.017    (1e-07)   -0.109    (3e-230)   0.140
work      :  -0.055    (4e-61)   -0.099    (5e-190)   0.092
achieve   :  -0.033    (2e-23)   -0.076    (2e-114)   0.081
money     :  -0.027    (2e-16)   -0.150    (0e+00)    0.139
relig     :   0.017    (2e-07)   -0.096    (1e-178)   0.136
death     :   0.001    (6e-01)   -0.163    (0e+00)    0.140





==> tables/del_user_attr_corr.tex <==
Category        :   r        p(r=0)     rho      p(rho=0)   mic
----------------------------------------------------------------
followers_count : -0.006   (6e-02)    -0.084    (3e-141)   0.039
tweet_rate      : -0.069   (8e-96)    -0.215    (0e+00)    0.086
friends_count   : -0.080   (1e-129)   -0.137    (0e+00)    0.031
listed_count    : -0.094   (3e-178)   -0.198    (0e+00)    0.047


==> tables/delphoto-stats.tex <==
\begin{table}
\centering
\begin{tabu} to \linewidth{@{}lX[r]X[r]X[r]X[r]@{}}
\toprule

& \mca{Deleted Tweet Set} & \mca{Regular Tweet Set} \\

\rowfont[c]{}
& Status Update & Direct Message & Status Update & Direct Message \\

\midrule

Twitter   & 68.94\% & 92.24\% & 20.59\% & 18.48\% \\
Instagram & 69.08\% & 51.09\% & 38.62\% & 23.21\% \\
Facebook  & 27.48\% & 57.57\% & 18.89\% & 15.15\% \\
Vine      & 22.51\% & 37.36\% & 13.65\% & 23.03\% \\

\bottomrule
\end{tabu}
\caption{Percentage of tweets
containing a link to media
hosted at Twitter, Instagram, Facebook, and Vine
for which the media was removed from the hosting site.
For example,
of all the update tweets in the deleted tweet set,
that contained a link to an instagram photo,
for 69.08\% of these tweets,
the photo that the tweet linked to
has been removed from Instagram.}
\label{tab:delphoto-stats}
\end{table}



==> tables/formality-cmp.tex <==
\begin{table}
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabu} to \linewidth{@{}lrrr@{}}
\toprule

\rowfont[c]{}
& AggDiff & DelUsers & NonDelUsers \\

\midrule

Character Count  &  & 15.11\% & 13.32\% \\
Word Count       &  & 15.06\% & 11.61\% \\
Dictionary Words &  & 20.68\% & 10.15\% \\
Lexical Density  &  & 5.21\%  & 12.28\% \\

\bottomrule
\end{tabu}
\caption{Difference in deleted and non-deleted tweet construction,
  with respect to size, lexical density, and use of dictionary words.}
\label{tab:formality-cmp}
\end{table}

% Signifcance level
% Char count : 2,983 (15.112%)    2,631 (13.329%) 19,739
% Word count : 2,974 (15.067%)    2,293 (11.617%) 19,739
% Lexical Density : 1,029 (5.213%)     2,424 (12.28%)  19,739
% Dictionary words : 4,083 (20.685%)    2,005 (10.158%) 19,739

% project_deltweets/data/tweet_dict_frac_dist_nondel.txt.gz
% N: 11,429,663, Mean: 0.723675, Median: 0.75, Std: 0.202049
% project_deltweets/data/tweet_dict_frac_dist_nonsupdel.txt.gz
% N: 1,210,434, Mean: 0.743825, Median: 0.785714, Std: 0.202708
% project_deltweets/data/tweet_len_dist_nondel.txt.gz
% N: 11,429,663, Mean: 63.2471, Median: 54, Std: 36.6202
% project_deltweets/data/tweet_len_dist_nonsupdel.txt.gz
% N: 1,210,434, Mean: 58.5338, Median: 50, Std: 34.5753
% project_deltweets/data/tweet_lexical_density_dist_nondel.txt.gz
% N: 11,429,663, Mean: 0.559053, Median: 0.55, Std: 0.160006
% project_deltweets/data/tweet_lexical_density_dist_nonsupdel.txt.gz
% N: 1,210,434, Mean: 0.550904, Median: 0.541667, Std: 0.164424
% project_deltweets/data/tweet_token_count_dist_nondel.txt.gz
% N: 11,429,663, Mean: 11.3596, Median: 9, Std: 7.13657
% project_deltweets/data/tweet_token_count_dist_nonsupdel.txt.gz
% N: 1,210,434, Mean: 10.7611, Median: 9, Std: 6.91531


==> tables/good-nort-mentioned-diff.tex <==
\begin{table}
\centering
\setlength{\tabcolsep}{4pt}
\begin{tabu} to \linewidth{@{}lrr@{}}
\toprule

& Deleted Tweet Set & Regular Tweet Set\\

\midrule

\# Users           & 395,599         & 647,213         \\
Median Followers   & 585             & 542             \\
Median Followees   & 361             & 377             \\
Median Tweet Rate  & 9.17 tweets/day & 9.13 tweets/day \\
Median Account Age & 916 days        & 984 days        \\
Accounts with Bio  & 92.01\%        & 93.05\%        \\
Accounts with Url  & 33.33\%        & 35.42\%        \\

\bottomrule
\end{tabu}
\caption{Summary statistics of the attributes of users
  who are mentioned in the deleted tweets set
  and the regular tweets dataset.}
\label{tab:good-nort-mentioned-diff}
\end{table}

% D: data/good-nort-mentioned-users/del-origtweets-replies-good-activity_period.txt
% N: 395,598, Mean: 8.33252e+07, Median: 7.91344e+07, Std: 5.48975e+07
% %: 5: 5.6612e+06, 10: 1.27004e+07, 25: 3.65049e+07
% %: 75: 1.20171e+08, 90: 1.68421e+08, 95: 1.77208e+08
% D: data/good-nort-mentioned-users/rand-origtweets-replies-good-activity_period.txt
% N: 647,213, Mean: 8.83218e+07, Median: 8.50019e+07, Std: 5.52861e+07
% %: 5: 7.07449e+06, 10: 1.5579e+07, 25: 4.16299e+07
% %: 75: 1.28577e+08, 90: 1.71089e+08, 95: 1.78423e+08
% MWU: u = 1.21258e+11, p = 0
% KS 2 Samp: Dnn = 0.0388063, p = 9.7825e-322

% D: data/good-nort-mentioned-users/del-origtweets-replies-good-created_at.txt
% N: 395,598, Mean: 1.33147e+09, Median: 1.33567e+09, Std: 5.48975e+07
% %: 5: 1.23759e+09, 10: 1.24638e+09, 25: 1.29463e+09
% %: 75: 1.3783e+09, 90: 1.4021e+09, 95: 1.40914e+09
% D: data/good-nort-mentioned-users/rand-origtweets-replies-good-created_at.txt
% N: 647,213, Mean: 1.32648e+09, Median: 1.3298e+09, Std: 5.52861e+07
% %: 5: 1.23638e+09, 10: 1.24371e+09, 25: 1.28622e+09
% %: 75: 1.37317e+09, 90: 1.39922e+09, 95: 1.40773e+09
% MWU: u = 1.21258e+11, p = 0
% KS 2 Samp: Dnn = 0.0388063, p = 9.7825e-322

% D: data/good-nort-mentioned-users/del-origtweets-replies-good-followers_count.txt
% N: 395,599, Mean: 27435.3, Median: 585, Std: 387378
% %: 5: 39, 10: 88, 25: 239
% %: 75: 1,952, 90: 14,144.2, 95: 50,017.1
% D: data/good-nort-mentioned-users/rand-origtweets-replies-good-followers_count.txt
% N: 647,212, Mean: 18739.2, Median: 542, Std: 305701
% %: 5: 43, 10: 90, 25: 229
% %: 75: 1,622, 90: 9,011, 95: 29,734.9
% MWU: u = 1.23978e+11, p = 6.99534e-162
% KS 2 Samp: Dnn = 0.0264107, p = 2.98408e-149

% D: data/good-nort-mentioned-users/del-origtweets-replies-good-friends_count.txt
% N: 395,592, Mean: 1572.68, Median: 361, Std: 11623
% %: 5: 38, 10: 78, 25: 177
% %: 75: 760, 90: 1,833, 95: 3,544
% D: data/good-nort-mentioned-users/rand-origtweets-replies-good-friends_count.txt
% N: 647,202, Mean: 1429.46, Median: 377, Std: 10090.6
% %: 5: 47, 10: 88, 25: 189
% %: 75: 792, 90: 1,866, 95: 3,285
% MWU: u = 1.24816e+11, p = 3.00893e-102
% KS 2 Samp: Dnn = 0.0188747, p = 1.95206e-76

% D: data/good-nort-mentioned-users/del-origtweets-replies-good-statuses_count.txt
% N: 395,599, Mean: 18030.9, Median: 7023, Std: 31435.2
% %: 5: 84, 10: 285, 25: 1,624
% %: 75: 21,507.5, 90: 48,132.2, 95: 72,299.1
% D: data/good-nort-mentioned-users/rand-origtweets-replies-good-statuses_count.txt
% N: 647,212, Mean: 18142.5, Median: 7517, Std: 30865.2
% %: 5: 133, 10: 408, 25: 1,964
% %: 75: 21,762, 90: 47,628, 95: 71,517.9
% MWU: u = 1.24884e+11, p = 2.55696e-98
% KS 2 Samp: Dnn = 0.0259391, p = 5.51976e-144

% D: data/good-nort-mentioned-users/del-origtweets-replies-good-statuses_per_day.txt
% N: 395,599, Mean: 20.2822, Median: 9.17393, Std: 34.022
% %: 5: 0.330833, 10: 0.814814, 25: 2.84116
% %: 75: 24.7696, 90: 51.5771, 95: 75.5591
% D: data/good-nort-mentioned-users/rand-origtweets-replies-good-statuses_per_day.txt
% N: 647,210, Mean: 19.9216, Median: 9.1311, Std: 33.4255
% %: 5: 0.4005, 10: 0.915944, 25: 2.95608
% %: 75: 24.1819, 90: 50.2947, 95: 73.9565
% MWU: u = 1.27771e+11, p = 0.0490303
% KS 2 Samp: Dnn = 0.00944464, p = 1.85657e-19

% * deleted set # users : 395,599
% * random set # users : 647,213

% * deleted set # users with bio : 364,019 / 395,599 = 92.0172%
% * random set # users with bio  : 602,285 / 647,213 = 93.0582%
% Fisher-Exact: OR = 0.859858, p = 2.79883e-86

% * deleted set # users with url : 131,886 / 395,599 = 33.3383%
% * random set # users with url  : 229,266 / 647,213 = 35.4236%
% Fisher-Exact: OR = 0.911693, p = 8.2885e-105



==> tables/good-retweeted-user-diff.tex <==
\begin{table}
\centering
\setlength{\tabcolsep}{4pt}
\begin{tabu} to \linewidth{@{}lrr@{}}
\toprule

& Deleted Tweet Set & Regular Tweet Set \\

\midrule

\# Users           & 326,400 & 452,009 \\
Median Followers   & 887             & 934 \\
Median Followees   & 432             & 472 \\
Median Tweet Rate  & 11.7 tweets/day & 11.4 tweets/day \\
Median Account Age & 868 days        & 958 days \\
Accounts with Bio  & 89.25\% & 91.43\% \\
Accounts with Url  & 33.25\% & 39.18\% \\

\bottomrule
\end{tabu}
\caption{Summary statistics of the attributes of users
who are retweeted in the deleted tweet set and the regular tweets dataset.}
\label{tab:good-retweeted-user-diff}
\end{table}

% del retweeted users : 326,400
% rand retweeted users : 452,009

% D: data/good-retweeted-users/del-followers_count.txt
% N: 326,400, Mean: 29669.3, Median: 887.5, Std: 410859
% %: 5: 67, 10: 143, 25: 355
% %: 75: 3,408, 90: 20,353.1, 95: 60,355.5
% D: data/good-retweeted-users/rand-followers_count.txt
% N: 452,009, Mean: 26189.1, Median: 934, Std: 358815
% %: 5: 75, 10: 151, 25: 365
% %: 75: 3,716, 90: 19,881.2, 95: 56,264.8
% KS 2 Samp: Dnn = 0.0159377, p = 2.89008e-42
% MWU: u = 7.26595e+10, p = 4.69121e-30

% D: data/good-retweeted-users/del-friends_count.txt
% N: 326,385, Mean: 2543.94, Median: 432, Std: 14768.4
% %: 5: 38, 10: 85, 25: 202
% %: 75: 982, 90: 3,068, 95: 8,466
% D: data/good-retweeted-users/rand-friends_count.txt
% N: 451,997, Mean: 2413.57, Median: 472, Std: 13450.2
% %: 5: 47, 10: 96, 25: 222
% %: 75: 1,090, 90: 3,159, 95: 7,927.2
% KS 2 Samp: Dnn = 0.0314423, p = 2.90102e-163
% MWU: u = 7.08073e+10, p = 8.87012e-201

% D: data/good-retweeted-users/del-statuses_per_day.txt
% N: 326,400, Mean: 23.2138, Median: 11.7694, Std: 35.642
% %: 5: 0.348376, 10: 0.894963, 25: 3.53444
% %: 75: 29.7211, 90: 57.8184, 95: 82.3103
% D: data/good-retweeted-users/rand-statuses_per_day.txt
% N: 452,009, Mean: 23.3773, Median: 11.4881, Std: 36.7809
% %: 5: 0.465299, 10: 1.05137, 25: 3.56467
% %: 75: 29.5072, 90: 58.4131, 95: 83.6231
% KS 2 Samp: Dnn = 0.0128142, p = 1.79463e-27
% MWU: u = 7.37617e+10, p = 0.48217

% D: data/good-retweeted-users/del-activity_period.txt
% N: 326,400, Mean: 7.89422e+07, Median: 7.49819e+07, Std: 5.25546e+07
% %: 5: 5.27599e+06, 10: 1.17788e+07, 25: 3.40509e+07
% %: 75: 1.13815e+08, 90: 1.61186e+08, 95: 1.74499e+08
% D: data/good-retweeted-users/rand-activity_period.txt
% N: 452,009, Mean: 8.63373e+07, Median: 8.27969e+07, Std: 5.42079e+07
% %: 5: 7.44724e+06, 10: 1.57087e+07, 25: 4.04199e+07
% %: 75: 1.23174e+08, 90: 1.69007e+08, 95: 1.77492e+08
% KS 2 Samp: Dnn = 0.0515901, p = 0
% MWU: u = 6.80592e+10, p = 0

% del retweeted Users with bio : 291,320 / 326,400 = 89.2525%
% rand retweeted users with bio : 413,287 / 452,009 = 91.4334%
% Fisher-Exact: OR = 0.778067, p = 2.4461e-228

% del retweeted Users with url : 108,559 / 326,400 = 33.2595%
% rand retweeted users with url : 177,124 / 452,009 = 39.1859%
% Fisher-Exact: OR = 0.773392, p = 0


==> tables/good-tweet-diff.tex <==
\begin{table}
\centering
\setlength{\tabcolsep}{4pt}
\begin{tabu} to \linewidth{@{}lrr@{}}
\toprule

& Deleted Tweet Set & Regular Tweet Set\\

\midrule

\# Tweets             & 2,893,127          & 2,813,732          \\
\# Retweets           & 1,496,488 (51.7\%) & 1,183,561 (42.0\%) \\
\# Replies            & 374,099   (12.9\%) & 557,201 (19.8\%)   \\
\# Tweets w/ hashtags & 350,817   (12.1\%) & 466,152 (16.5\%)   \\
\# Tweets w/ mentions & 2,021,169 (69.8\%) & 1,945,235 (69.1\%) \\
\# Tweets w/ urls     & 408,315   (14.1\%) & 397,424 (14.1\%)   \\
\# Tweets w/ location & 45,453    (1.57\%) & 58,634 (2.08\%)    \\
\bottomrule
\end{tabu}
\caption{Summary statistics of tweet attributes
in the deleted tweet set and the regular tweets dataset.}
\label{tab:good-tweet-diff}
\end{table}

% 350,817   / 2,893,127 =  12.1259%
% 466,152   /  2,813,732 =  16.567%
% Fisher-Exact: OR = 0.694936, p = 0

% 2,021,169 / 2,893,127 =  69.8611%
% 1,945,235 /  2,813,732 =  69.1336%
% Fisher-Exact: OR = 1.03491, p = 2.04345e-79

% 408,315   / 2,893,127 =  14.1133%
% 397,424   /  2,813,732 =  14.1244%
% Fisher-Exact: OR = 0.999079, p = 0.702227

% 45,453    / 2,893,127 =  1.57107%
% 58,634    /  2,813,732 =  2.08385%
% Fisher-Exact: OR = 0.749997, p = 0

% 1,496,488 / 2,893,127 =  51.7256%
% 1,183,561 /  2,813,732 =  42.0637%
% Fisher-Exact: OR = 1.47581, p = 0

% 374,099   / 2,893,127 =  12.9306%
% 557,201   /  2,813,732 =  19.8029%
% Fisher-Exact: OR = 0.601427, p = 0


==> tables/lang-del-diff-pos.tex <==
\begin{table}
\centering
\setlength{\tabcolsep}{4pt}
\begin{tabu} to \linewidth{@{}lrr@{}}
\toprule

& Deleters & Non Deleters \\

\midrule

\# Users            & 106,965         & 101,137 \\
Median Followers    & 502             & 355 \\
Median Followees    & 402             & 386 \\
Median Listed Count & 2               & 2 \\
Median Tweet Rate   & 8.72 tweets/day & 4.37 tweets/day\\
Accounts with Bio   & 88.60\%         & 87.22\% \\
Accounts with Url   & 28.82\%         & 35.08\% \\

\bottomrule
\end{tabu}
\caption{Summary statistics of the user attributes
for users in the deleter and the non-deleter sets.}
\label{tab:user-diff}
\end{table}

% D: data/lang-del-diff/pos-proper_noun.txt
% N: 85,340, Mean: 1.18173, Median: 0.0869565, Std: 8.74219
% %: 5: -1, 10: -0.826326, 25: -0.383505
% %: 75: 0.780055, 90: 1.90804, 95: 3.14286

% D: data/lang-del-diff/pos-common_noun.txt
% N: 85,340, Mean: 0.403064, Median: 0.143518, Std: 3.70493
% %: 5: -0.517857, 10: -0.367931, 25: -0.130917
% %: 75: 0.5, 90: 1.01136, 95: 1.4812

% D: data/lang-del-diff/pos-verb.txt
% N: 85,340, Mean: 0.464949, Median: 0.119142, Std: 3.99803
% %: 5: -0.557114, 10: -0.397946, 25: -0.151814
% %: 75: 0.477778, 90: 1.07071, 95: 1.74623

% D: data/lang-del-diff/pos-adjective.txt
% N: 85,340, Mean: 0.676417, Median: 0.0384615, Std: 6.53715
% %: 5: -1, 10: -0.609837, 25: -0.294534
% %: 75: 0.484848, 90: 1.17859, 95: 2

% D: data/lang-del-diff/pos-adverb.txt
% N: 85,340, Mean: 0.861956, Median: 0.0528166, Std: 7.54068
% %: 5: -1, 10: -0.639596, 25: -0.298246
% %: 75: 0.52381, 90: 1.31916, 95: 2.31183

% D: data/lang-del-diff/pos-mention.txt
% N: 85,340, Mean: 3.03583, Median: 0.634937, Std: 25.3226
% %: 5: -0.612813, 10: -0.333333, 25: 0.0707118
% %: 75: 1.74286, 90: 4.18529, 95: 7.875

% D: data/lang-del-diff/pos-hashtag.txt
% N: 85,340, Mean: 9.56006, Median: 0, Std: 28.5182
% %: 5: -1, 10: -1, 25: -1
% %: 75: 1.55556, 90: 16.2327, 95: 100

% D: data/lang-del-diff/pos-url.txt
% N: 85,340, Mean: 5.71119, Median: 1.25, Std: 17.9142
% %: 5: -1, 10: -0.402795, 25: 0.178571
% %: 75: 3.44726, 90: 8.55556, 95: 18.6208

% D: data/lang-del-diff/pos-emoticon.txt
% N: 85,340, Mean: 3.23326, Median: -0.333333, Std: 17.5678
% %: 5: -1, 10: -1, 25: -1
% %: 75: 0.261521, 90: 2.02922, 95: 6.15397

% D: data/lang-del-diff/pos-lexical_density.txt
% N: 85,340, Mean: -0.076972, Median: -0.0901716, Std: 0.868251
% %: 5: -0.304711, 10: -0.248983, 25: -0.170536
% %: 75: -0.00953559, 90: 0.0788727, 95: 0.148251


==> tables/origtweet-hashtag-discrepency.tex <==
\begin{table}
\begin{tabu} to \linewidth{@{}lX[l]@{}}
\toprule

Topic & Hashtags \\

\midrule

Cursing & Scum, Whore, GetOut \\
Photos & KikMeBoys, InstaRepost \\
Jobs & OnlineOpportunity, HomeBusinessesIdeas \\
Marketing & LikeHero, BestAffiliateWebsites, OnlineAffiliatePrograms \\
Others & FilmesGR, TweetCleaning \\

\bottomrule
\end{tabu}
% \caption{Hashtags that were popular in the deleted tweet set,
% but were significantly less popular in the regular tweet set.}
\caption{Top hashtags in the deleted tweet set,
with highest rank loss in the regular tweet set.}
\label{tab:del-origtweet-hashtag-discrepency}
\end{table}

\begin{table}
\begin{tabu} to \linewidth{@{}lX[l]@{}}
\toprule

Topic & Hashtags \\

\midrule

Music & CriaturaEmocional, Evanescence, InfiniteF \\
Acting & PabloMartinez, SanayaSexyIrani, SukirtiKandpal, LaliEsposito \\
Voting & DWTSBethanyArtem, DWTSLeaTony AllAboutThatBassEMA \\
Politics & IsBailNotMeant4HinduSaints, GoveGone \\
Celebrity Fans & KatyPerrySexiest, ILoveYou1DFandom \\

\bottomrule
\end{tabu}
\caption{Top hashtags in the regular tweet set,
with highest rank loss in deleted Tweet set.}
\label{tab:rand-origtweet-hashtag-discrepency}
\end{table}

% Deleted Tweet Hashtags
% ----------------------
% kikmeboys : 1368.5 : 132141.5 : 9555.93715747 | Kick me boys - 
% filmesgr : 11.0 : 1041.0 : 9363.63636364 | AssistirFilmesOnline.com - Pirated movies online
% tweetcleaning : 1652.5 : 132141.5 : 7896.45990923 | Tweet Cleaning
% - asksteven : 2053.0 : 132141.5 : 6336.50754993 | StevenFhoney - bad post
% instarepost : 2196.0 : 132141.5 : 5917.37249545 | Posts to instagram videos
% - championshipshyvana : 2507.0 : 132141.5 : 5170.90147587 | League of legends related
% onlineopportunity : 2555.0 : 132141.5 : 5071.87866928 | jobs
% homebusinessesideas : 2555.0 : 132141.5 : 5071.87866928 | jobs
% likehero : 1319.0 : 66757.0 : 4961.18271418 | marketing 
% whore : 2756.5 : 132141.5 : 4693.81461999 | curseing
% - frfr : 2756.5 : 132141.5 : 4693.81461999 | for real for real
% scum : 2756.5 : 132141.5 : 4693.81461999 | cursing
% bestaffiliatewebsites : 2756.5 : 132141.5 : 4693.81461999 | marketing
% onlineaffiliateprograms : 3018.5 : 132141.5 : 4277.72072221 | marketing
% - wearekatycats : 3018.5 : 132141.5 : 4277.72072221 | katypary facs
% - viridian : 3018.5 : 132141.5 : 4277.72072221 | color, housing
% - callmedana : 3296.5 : 132141.5 : 3908.53935993 | dana white - ufc related
% - emabieggestfansjutinbieber : 3296.5 : 132141.5 : 3908.53935993 | justin beiber
% - visa : 3296.5 : 132141.5 : 3908.53935993 | visa
% getout : 3296.5 : 132141.5 : 3908.53935993 | cursing


% Random Tweet Hashtags
% ---------------------
% criaturaemocional : 249.0 : 114149.0 : 45742.9718876 | song
% pablomartinez : 322.0 : 114149.0 : 35350.0 | actor
% gonzalohiguain : 43.0 : 15092.5 : 34998.8372093 | football player
% - gigatowngis : 356.0 : 114149.0 : 31964.3258427 | palce
% IsBailNotMeant4HinduSaints : 372.0 : 114149.0 : 30585.2150538 | movement
% ILoveYou1dFandom : 528.5 : 114149.0 : 21498.6754967 | one direction
% sanayasexyirani : 537.0 : 114149.0 : 21156.7970205 | actress
% - \ubc31\uc77c\ubabd : 232.0 : 44540.5 : 19098.4913793 
% evanescence : 604.5 : 114149.0 : 18783.2092639 | band
% govegone : 714.5 : 114149.0 : 15876.0671798 | politician
% - lorenabueri : 773.5 : 114149.0 : 14657.4660633 | porn actress
% infinitef : 809.0 : 114149.0 : 14009.8887515 | sk band
% sukirtikandpal : 813.0 : 114149.0 : 13940.4674047 | actress
% -horortamanlangsatmayestik : 822.0 : 114149.0 : 13786.7396594
% allaboutthatbassema : 951.0 : 114149.0 : 11903.0494217 | song
% dwtsbethanyartem : 1018.0 : 114149.0 : 11113.064833 | voting
% laliesposito : 27.0 : 2981.5 : 10942.5925926 | acrtess
% katyperrysexiest : 1055.0 : 114149.0 : 10719.8104265 | artist
% dwtsleatony : 1056.5 : 114149.0 : 10704.4486512 | voting
% - tcretweet : 1060.0 : 114149.0 : 10668.7735849 | follow


==> tables/predict-all-heavy.tex <==
\begin{table}
\centering
\small

\begin{tabu} to \linewidth{@{}lrrrr@{}}
\toprule

\rowfont[c]{}
Classifier & Accuracy & Precision & Recall & F1-Score \\

\midrule

SVM & 0.675 & 0.861 & 0.723 & 0.786 \\
AdaBoost & 0.798 & 0.881 & 0.876 & 0.876 \\

\bottomrule
\end{tabu}
\caption{Classifier performance in distinguising
  deleted tweets from non-deleted tweets
  using only open text features,
  all post time features,
and all post time as well as response features}
\label{tab:predict-all-heavy}
\end{table}

% SVM - Post Time features - Del10pc
%
% f1        : 0.78637413394919164
% pr_auc    : 0.89599075482581703
% recall    : 0.72331386086032923
% precision : 0.86148007590132825
% accuracy  : 0.67515364354697105
% roc_auc   : 0.64517300026217261

% AdaBoost - Post Time features - Del10pc
%
% f1        : 0.87867020074379998
% pr_auc    : 0.94155553578238083
% recall    : 0.87613194017619345
% precision : 0.88122321134190573
% accuracy  : 0.79892396227057583
% roc_auc   : 0.77675421917905729


==> tables/predict-open-text-all.tex <==
\begin{table}
\centering
\small

\begin{tabu} to \linewidth{@{}lrrr@{}}
\toprule

\rowfont[c]{}
Classifier & Precision & Recall & F1-Score \\

\midrule
\multicolumn{4}{l}{\textbf{Open text features only}} \\

Naive Bayes & 0.541 & 0.705 & 0.612 \\
Linear SVM  & 0.572 & 0.605 & 0.588 \\

\midrule
\multicolumn{4}{l}{\textbf{All post time features}} \\

SVM      & 0.630 (0.861) & 0.756 (0.723) & 0.687 (0.786) \\
AdaBoost & 0.796 (0.881) & 0.765 (0.876) & 0.780 (0.876) \\

% \midrule
% \multicolumn{4}{l}{\textbf{All post time and response features}} \\

% SVM      & 0.709 & 0.676 & 0.692 \\
% AdaBoost & 0.825 & 0.809 & 0.817 \\

\bottomrule
\end{tabu}
\caption{Classifier performance in distinguising
  deleted tweets from non-deleted tweets
  using only open text features,
  and all post time features,
and all post time as well as response features}
\label{tab:predict-open-text-all-late}
\end{table}

% LinearSVC Classifer - Open Text Features
%
% Final Classifier
% C = 1e-06
%
% f1        : 0.58831548493615471,
% pr_auc    : 0.5897784259087091,
% recall    : 0.60494673229082296,
% precision : 0.57257422531473889,
% accuracy  : 0.57498944471375624,
% roc_auc   : 0.60410182645887167

% Multinomial Naive Bayes Classifer - Open Text Features
%
% Final Classifer
% alpha=0.1
%
% f1         : 0.61280252969554472,
% pr_auc     : 0.6539167689191967,
% recall     : 0.70519080645662924,
% precision  : 0.54181800802905755,
% accuracy   : 0.5521499241938761,
% roc_auc    : 0.56281877302426531


==> tables/sent-cmp.tex <==
\begin{table}
\centering
\setlength{\tabcolsep}{1pt}
\begin{tabu} to \linewidth{@{}lX[r]X[r]X[r]@{}}
\toprule

\rowfont[c]{}
& Deleted Tweets & Non-Deleted Tweets & Difference \\

\midrule

\% of +ve tweets & 56.52\% & 61.76\% & -8.47\% \\
\% of -ve tweets & 43.47\% & 38.23\% & 13.68\% \\

\bottomrule
\end{tabu}
\caption{Comparison of the percentage of tweets containing
poistive and negative sentiments
in the deleted and non-deleted tweet sets.}
\label{tab:sent-cmp}
\end{table}


==> tables/suspended-user-diff.tex <==
\begin{table}
\centering
\setlength{\tabcolsep}{4pt}
\begin{tabu} to \linewidth{@{}lrr@{}}
\toprule

& Deleted Tweet Set & Regular Tweet Set\\

\midrule

\# Users           & 49,621 (2.66\%) & 46,254 (1.89\%) \\
Median Followers   & 0 & 5 \\
Median Followees   & 1 & 38 \\
Median Tweet Rate  & 2.00 tweets/day & 2.94 tweets/day \\
Median Account Age & 13 days & 48 days        \\
Accounts with Bio  & 39.65\% & 50.55\% \\
Accounts with Url  & 6.63\% & 1.64\% \\

\bottomrule
\end{tabu}
\caption{Summary statistics of the attributes of suspended users
  in the deleted tweet set and the regular tweet set.}
\label{tab:suspended-user-diff}
\end{table}

% D: data/users/suspended/del-suspended-activity_period.txt
% N: 49,621, Mean: 1.2028e+07, Median: 1.12818e+06, Std: 2.27002e+07
% %: 5: 7,633, 10: 13,054, 25: 23,509
% %: 75: 1.65102e+07, 90: 3.09349e+07, 95: 4.17226e+07
% D: data/users/suspended/rand-suspended-activity_period.txt
% N: 46,254, Mean: 1.46617e+07, Median: 4.1585e+06, Std: 2.58777e+07
% %: 5: 23,467, 10: 143,029, 25: 901,880
% %: 75: 1.62813e+07, 90: 3.75206e+07, 95: 7.99314e+07
% MWU: u = 9.12761e+08, p = 0
% KS 2 Samp: Dnn = 0.30785, p = 0

% D: data/users/suspended/del-suspended-created_at.txt
% N: 49,621, Mean: 1.40139e+09, Median: 1.41216e+09, Std: 2.24213e+07
% %: 5: 1.37262e+09, 10: 1.38271e+09, 25: 1.39688e+09
% %: 75: 1.41267e+09, 90: 1.41327e+09, 95: 1.4137e+09
% D: data/users/suspended/rand-suspended-created_at.txt
% N: 46,254, Mean: 1.39926e+09, Median: 1.40947e+09, Std: 2.57568e+07
% %: 5: 1.33445e+09, 10: 1.37654e+09, 25: 1.39736e+09
% %: 75: 1.41275e+09, 90: 1.41353e+09, 95: 1.4141e+09
% MWU: u = 1.10391e+09, p = 1.00844e-24
% KS 2 Samp: Dnn = 0.169786, p = 0

% D: data/users/suspended/del-suspended-followers_count.txt
% N: 49,621, Mean: 3198.01, Median: 0, Std: 12428.3
% %: 5: 0, 10: 0, 25: 0
% %: 75: 1,973, 90: 11,840, 95: 19,118
% D: data/users/suspended/rand-suspended-followers_count.txt
% N: 46,254, Mean: 1217.17, Median: 5, Std: 7511.94
% %: 5: 0, 10: 0, 25: 0
% %: 75: 146, 90: 1,016, 95: 7,451
% KS 2 Samp: Dnn = 0.172822, p = 0
% MWU: u = 1.13546e+09, p = 0.00231339

% D: data/users/suspended/del-suspended-friends_count.txt
% N: 49,621, Mean: 2747.77, Median: 1, Std: 5562.03
% %: 5: 0, 10: 0, 25: 0
% %: 75: 1,851, 90: 10,139, 95: 16,472
% D: data/users/suspended/rand-suspended-friends_count.txt
% N: 46,254, Mean: 883.886, Median: 38, Std: 4242.28
% %: 5: 0, 10: 0, 25: 0
% %: 75: 210, 90: 1,264, 95: 6,097.4
% KS 2 Samp: Dnn = 0.228534, p = 0
% MWU: u = 1.06747e+09, p = 2.07779e-78

% D: data/users/suspended/del-suspended-statuses_count.txt
% N: 49,108, Mean: 2193.43, Median: 62, Std: 13091.7
% %: 5: 1, 10: 1, 25: 2
% %: 75: 412, 90: 1,065, 95: 10,035.1
% D: data/users/suspended/rand-suspended-statuses_count.txt
% N: 46,177, Mean: 6657.71, Median: 143, Std: 28564.1
% %: 5: 1, 10: 4, 25: 25
% %: 75: 1,192, 90: 18,662.6, 95: 25,475
% MWU: u = 8.48923e+08, p = 0
% KS 2 Samp: Dnn = 0.230484, p = 0

% D: data/users/suspended/del-suspended-statuses_per_day.txt
% N: 49,108, Mean: 14.5011, Median: 2, Std: 50.1643
% %: 5: 0.333234, 10: 1, 25: 1
% %: 75: 4.4709, 90: 32.2347, 95: 82.0485
% D: data/users/suspended/rand-suspended-statuses_per_day.txt
% N: 46,177, Mean: 36.9132, Median: 3.94166, Std: 106.92
% %: 5: 0.119188, 10: 0.305371, 25: 1.0867
% %: 75: 23.8928, 90: 98.593, 95: 146.38
% KS 2 Samp: Dnn = 0.241381, p = 0
% MWU: u = 9.28545e+08, p = 0

% * users with bio del-suspended  : 19677 / 49621 = 39.6546%
% * users with bio rand-suspended : 23381 / 46254 = 50.5491%
% Fisher-Exact: OR = 0.642849, p = 4.68776e-252

% * users with url del-suspended  : 3,291 / 49621 = 6.63227%
% * users with url rand-suspended :  7,61 / 46254 = 1.64526%
% Fisher-Exact: OR = 4.24644, p = 0


==> tables/tweet-time-categorize.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{1.5pt}
\begin{tabu} to \linewidth{@{}lrrrr@{}}
\toprule

& Hour & Day & Week & Month \\

\midrule

Reveal too much    & 28 & 46 & 37 & 42 \\
Expressive         & 20 & 30 & 36 & 33 \\
Direct attack      & 2  & 6  & 0  & 8  \\
Blunder            & 3  & 3  & 4  & 3  \\
Behavior edict     & 12 & 17 & 8  & 18 \\

\midrule

Offensive comments & 11 & 13 & 13 & 11 \\
Sexual activity    & 2  & 4  & 1  & 0  \\
Alcohol/drug use   & 0  & 0  & 1  & 2  \\

% Follow Requests    & 3  & 2  & 1  & 2  \\
% Relationship       & 5  & 8  & 5  & 2  \\
% Quote              & 1  & 1  & 7  & 7  \\
% Regrettable        & 0  & 3  & 1  & 1  \\

\bottomrule
\end{tabu}
\caption{Number of status updates (out of 100),
  deleted within an hour, a day, a week, and a month
  of their creation, which fall under
a given category according to majority decesion of the annotators
classifying the tweet.}
\label{tab:tweet-time-categorize}
\end{table}

% 28 20 2 3 12 11 2 0 3 5 1 0 / 100
% 46 30 6 3 17 13 4 0 2 8 1 3 / 100

% Fisher-Exact: OR = 0.456522 0.583333 0.319728 1 0.665775 0.827139 0.489796 nan 1.51546 0.605263 1 0
% Fisher-Exact: p = 0.0125311 0.141207 0.279043 1 0.42221 0.828211 0.682717 1 1 0.567925 1 0.246231

% 46 30 6 3 17 13 4 0 2 8 1 3  / 100
% 37 36 0 4 8 13 1 1 1 5 7 1 / 100

% Fisher-Exact: OR = 1.45045 0.761905 inf 0.742268 2.35542 1 4.125 0 2.02041 1.65217 0.134199 3.06186
% Fisher-Exact: p = 0.250872 0.452247 0.0289303 1 0.0856228 1 0.368671 1 1 0.567925 0.0648594 0.621202

% 37 36 0 4 8 13 1 1 1 5 7 1 / 100
% 42 33 8 3 18 11 0 2 2 2 7 1  / 100

% Fisher-Exact: OR = 0.811036 1.14205 0 1.34722 0.396135 1.20899 inf 0.494949 0.494949 2.57895 1 1
% Fisher-Exact: p = 0.563003 0.766214 0.00675467 1 0.0568471 0.828211 1 1 1 0.444754 1 1


==> tables/unsafe-user-diff.tex <==

\begin{table}
\centering
\setlength{\tabcolsep}{4pt}
\begin{tabu} to \linewidth{@{}lrr@{}}
\toprule

& Deleted Tweet Set & Regular Tweet Set\\

\midrule

\# Users           & 13,387 (0.72\%) & 6,153 (0.25\%) \\
Median Followers   & 11 & 165 \\
Median Followees   & 155 & 342 \\
Median Tweet Rate  & 0.59 tweets/day & 7.08 tweets/day \\
Median Account Age & 482 days & 184 days \\
Accounts with Bio  & 42.60\% & 60.78\% \\
Accounts with Url  & 14.00\% & 31.15\% \\

\bottomrule
\end{tabu}
\caption{Summary statistics of the attributes of users
  who have posted at-least one unsafe url
  in the deleted tweet set and the random tweet set.}
\label{tab:unsafe-user-diff}
\end{table}

% D: data/users/unsafe/del-unsafe-activity_period.txt
% N: 13,387, Mean: 5.54332e+07, Median: 4.16229e+07, Std: 4.69062e+07
% %: 5: 80, 10: 2.17629e+06, 25: 1.64487e+07
% %: 75: 8.9109e+07, 90: 1.23549e+08, 95: 1.47757e+08
% D: data/users/unsafe/rand-unsafe-activity_period.txt
% N: 6,153, Mean: 3.95009e+07, Median: 1.58845e+07, Std: 4.45667e+07
% %: 5: 810,955, 10: 2.0087e+06, 25: 1.08093e+07
% %: 75: 6.26101e+07, 90: 1.08825e+08, 95: 1.36761e+08
% MWU: u = 3.19175e+07, p = 1.42045e-141
% KS 2 Samp: Dnn = 0.273121, p = 1.40014e-274

% D: data/users/unsafe/del-unsafe-followers_count.txt
% N: 13,387, Mean: 4843.62, Median: 11, Std: 44931.6
% %: 5: 0, 10: 0, 25: 1
% %: 75: 379, 90: 7,573.8, 95: 20,592.1
% D: data/users/unsafe/rand-unsafe-followers_count.txt
% N: 6,153, Mean: 3086.54, Median: 165, Std: 22250
% %: 5: 0, 10: 0, 25: 5
% %: 75: 500, 90: 1,692.2, 95: 8,752.6
% KS 2 Samp: Dnn = 0.203668, p = 7.06407e-153
% MWU: u = 3.37563e+07, p = 8.74139e-92

% D: data/users/unsafe/del-unsafe-friends_count.txt
% N: 13,387, Mean: 2752.41, Median: 155, Std: 10935.7
% %: 5: 0, 10: 0, 25: 10
% %: 75: 1,226.5, 90: 6,661.8, 95: 17,147.1
% D: data/users/unsafe/rand-unsafe-friends_count.txt
% N: 6,153, Mean: 1898.04, Median: 342, Std: 9038.49
% %: 5: 0, 10: 1, 25: 15
% %: 75: 1,175, 90: 1,953, 95: 4,392.6
% KS 2 Samp: Dnn = 0.098625, p = 3.56737e-36
% MWU: u = 3.8872e+07, p = 1.33134e-10

% D: data/users/unsafe/del-unsafe-statuses_per_day.txt
% N: 13,355, Mean: 12.0472, Median: 0.596849, Std: 60.1629
% %: 5: 0.0200123, 10: 0.0389245, 25: 0.119368
% %: 75: 2.33079, 90: 13.05, 95: 38.339
% D: data/users/unsafe/rand-unsafe-statuses_per_day.txt
% N: 6,150, Mean: 60.0538, Median: 7.08533, Std: 107.702
% %: 5: 0.0428442, 10: 0.0899705, 25: 0.480583
% %: 75: 100.33, 90: 144.759, 95: 260.394
% MWU: u = 2.36673e+07, p = 0
% KS 2 Samp: Dnn = 0.359983, p = 0

% * users with bio del-unsafe :  5704 / 13387 = 42.6085% 
% * users with bio rand-unsafe : 3740 / 6153 = 60.7834% 
% Fisher-Exact: OR = 0.478999, p = 1.02087e-123

% * users with url del-unsafe :  1,873 / 13387  = 13.9912% 
% * users with url rand-unsafe  : 1,917 / 6153  = 31.1555% 
% Fisher-Exact: OR = 0.359456, p = 1.5801e-165


==> tables/user-diff.tex <==
\begin{table}
\centering
\setlength{\tabcolsep}{4pt}
\begin{tabu} to \linewidth{@{}lrr@{}}
\toprule

& Deleters & Non-Deleters \\

\midrule

\# Users            & 91,785          & 102,710 \\
Median Followers    & 508             & 375 \\
Median Followees    & 403             & 394 \\
Median Listed Count & 2               & 2 \\
Median Tweet Rate   & 8.85 tweets/day & 4.74 tweets/day\\
Accounts with Bio   & 88.43\%         & 88.08\% \\
Accounts with Url   & 27.88\%         & 35.32\% \\

\bottomrule
\end{tabu}
\caption{Summary statistics of the user attributes,
for users in the deleter and the non-deleter sets.}
\label{tab:user-diff}
\end{table}


% Users with non superficial deletions
% Num users: 91,785
% Median observed_tweets: 81.0
% Median friend count: 403.0
% Median follower count: 508.0
% Median listed count: 2.0
% Median activity rate: 8.85360264341 tweets/day
% Users with bio 81,168 88.43%
% Users with url 25,588 27.88%

% Users without non superficial deletions
% Num users: 102,710
% Median observed_tweets: 15.0
% Median friend count: 394.0
% Median follower count: 375.0
% Median listed count: 2.0
% Median activity rate: 4.74206947392 tweets/day
% Users with bio 90,468 88.08%
% Users with url 36,273 35.32%




==> tables/user-pos.tex <==
\begin{table}
\centering
\setlength{\tabcolsep}{4pt}
\begin{tabu} to \linewidth {@{}lrr@{}}
\toprule

& Deleters & Non-Deleters \\

\midrule

% Proper Noun & 0.38 & 0.63 \\
% Common Noun & 1.32 & 1.61 \\
% Verb        & 1.60 & 1.64 \\
% Adjective   & 0.53 & 0.60 \\
% Adverb      & 0.55 & 0.50 \\

% \midrule

Tweets w/ emoticons & 8.69\% & 3.57\% \\

\midrule

Tweets w/ mentions & 37.63\% & 35.63\% \\
Tweets w/ hashtags & 2.47\%  & 5.00\% \\
Tweets w/ urls     & 16.66\% & 29.03\% \\

\bottomrule
\end{tabu}
\caption{%
  % Median number of different part of speech tags used
% by individual users in the deleter and non-deleter sets.
Percentage of tweets with mentions, hashtags, urls,
and emoticons posted by individual users in the deleter and non-deleter
sets.}
\label{tab:user-pos}
\end{table}

% *               : del_users.pickle : *               : non_del_users.pickle
% # users         : 102701           : # users         : 80175
% proper_noun     : 0.385026737968   : proper_noun     : 0.633333333333
% common_noun     : 1.32894736842    : common_noun     : 1.6170212766
% verb            : 1.60606060606    : verb            : 1.64705882353
% adjective       : 0.531914893617   : adjective       : 0.6
% adverb          : 0.558139534884   : adverb          : 0.5
% mention         : 0.376383763838   : mention         : 0.35632183908
% hashtag         : 0.0247524752475  : hashtag         : 0.05
% url             : 0.166666666667   : url             : 0.290322580645
% emoticon        : 0.0869565217391  : emoticon        : 0.0357142857143
% lexical_density : 0.546806326484   : lexical_density : 0.546119086391



==> tables/user-sent.tex <==
\begin{table}
\centering
\setlength{\tabcolsep}{4pt}
\begin{tabu} to \linewidth {@{}lrrr@{}}
\toprule

& 10\% Deleters & Deleters & Non-Deleters \\

\midrule

Median \% of +ve~tweets & 63.41\% & 63.63\% & 69.23\% \\
Median \% of -ve~tweets & 36.58\% & 36.36\% & 29.16\% \\

\bottomrule
\end{tabu}
\caption{Comparison of the median percentage of tweets
with positive and negative sentiments posted by
the users in the deleter and non-deleter sets.}
\label{tab:user-sent}
\end{table}

% Sentiment
% *          : del users      : *          : non del users
% Median pos : 0.636363636364 : Median pos : 0.692307692308
% Median neg : 0.363636363636 : Median neg : 0.291666666667

% Del 10pc
% Median pos: 0.634146341463
% Median neg: 0.365853658537


